Iterative Row Sampling

There has been significant interest and progress recently in algorithms that solve regression problems involving tall and thin matrices in input sparsity time. These algorithms find shorter equivalent of a n*d matrix where n >> d, which allows one to solve a poly(d) sized problem instead. In practice, the best performances are often obtained by invoking these routines in an iterative fashion. We show these iterative methods can be adapted to give theoretical guarantees comparable and better than the current state of the art. Our approaches are based on computing the importances of the rows, known as leverage scores, in an iterative manner. We show that alternating between computing a short matrix estimate and finding more accurate approximate leverage scores leads to a series of geometrically smaller instances. This gives an algorithm that runs in $O(nnz(A) + d^{\omega + \theta} \epsilon^{-2})$ time for any $\theta > 0$, where the $d^{\omega + \theta}$ term is comparable to the cost of solving a regression problem on the small approximation. Our results are built upon the close connection between randomized matrix algorithms, iterative methods, and graph sparsification.

==> background.tex <==
\section{Background}
\label{sec:background}

In this section we outline key results from previous works on row sampling.
These works show that statistical leverage scores are closely
associated the probabilities needed for row sampling,
and give algorithms that efficiently approximate these values.
In addition, we formalize the observation implicit in earlier works
that both the sampling and estimation algorithms are very robust.
The high error-tolerance of these algorithms makes them ideal
as core routines to build iterative algorithms upon.
Most of the results mentioned in this section are direct adaptations
from earlier works, where they're presented in much more detail.
For completeness, we give their proofs in Appendix \ref{sec:backgroundproofs}.


Most of the presentation will use standard linear algebraic notations.
We use $||\vecx||_p$ to denote the $L_p$ norm of a vector.
The two values of $p$ that we'll use are $p=1$ and $p=2$,
which correspond to $||\vecx||_1 = \sum_{i} |x_i|$
and $||\vecx||_2 = \sqrt{\sum_{i} x_i^2}$.
For two vectors $\vecx$ and $\vecy$, $\vecx \geq \vecy$ means
$\vecx$ is entry-wise greater or equal to $\vecy$, aka.
$\vecx_i \geq \vecy_i$ for all $i$.
Given a matrix $\mata$, we use $\mata_{i, :}$, or $\veca_i$
to denote the $i^{th}$ row of $\mata$.
Note that $\veca_i$ is a row vector of length $d$.
We will also use its Forbenius norm, $||\mata||_F$
to denote the $2$-norm of all its entries.
Formally, $||\mata||_F^2 = \sqrt{\sum_{i, j} \mata_{i, j}^2}$.

The spectral theorem states that any symmetric matrix
$\matc$ has a full complement of orthonormal eigenvectors.
Let them and their eigenvalues
be $(\vecu_1, \lambda_1), (\vecu_2, \lambda_2), \ldots (\vecu_n, \lambda_n)$.
Here $\vecu_j$ is a length $d$ column vector, $\lambda_j$ is a scalar
and they satisfy $\mata^T \mata \vecu_j = \lambda_j \vecu_j$.
Without loss of generality we assume that $\lambda_j$s are in increasing
order: $\lambda_1 \leq \lambda_2 \leq \ldots \leq \lambda_n$.
Then if $\lambda_{k}$ is the first non-zero eigenvalue, we have:
\begin{align*}
\matc = \sum_{j = k}^{n} \lambda_j \vecu_j \vecu_j^T
\end{align*}
We will use $\lambda_{\max}$ to denote the largest eigenvalue,
and $\lambda_{\min}$ to denote the smallest \textbf{non-zero} eigenvalue.
Suppose $\lambda_k$ is the first non-zero eigenvalue,
the pseudoinverse of $\matc$, $\matc^{+}$ can be defined as:
\begin{align*}
\matc^{+} = \sum_{j = k}^{n} \frac{1}{\lambda_j} \vecu_j \vecu_j^T
\end{align*}
This is a linear operator that preserves the null space of $\matc$,
while acting as its inverse on the rank space.
A matrix $\matc$ is positive semi-definite
if all its eigenvalues are non-negative,
or equivalently $\vecx^T \matc \vecx \geq 0$
for all vectors $\vecx$.
Similarities between matrices is defined using a partial order on matrices.
Given two matrices $\mata$ and $\matb$, $\mata \preceq \matb$
denotes that $\matb - \mata$ is positive semi-definite.

We will use $\elementsum$ to specifically to denote $\mata^T \mata$.
An alternate view of row sampling is that we're given $n$
PSD matrices $\element_1 \ldots \element_n$
where $\element_i = \veca_i^T \veca_i$;
and the goal is to find a small subset of them such
that their weighted sum is close to $\elementsum$.
Furthermore, we can assign weights of zero to elements
that are not selected, giving a weight vector $\weightv \in \Re^{n}$.
The formal requirement of row sampling can be described as:

\begin{itemize}
\item For some parameter $\kappa$ we have $\elementsum
\preceq \sum_{i = 1}^n \weight_i \element_i
\preceq \kappa \elementsum$

\item  $|\{ i: w_i \neq 0\}|$, the support of $\vecw$, is small.
\end{itemize}

The work by Clarkson and Woodruff \cite{ClarksonW12} obtained
approximations to $\mata$ by applying a (randomized) linear
transformation $\mats$ to get $\matb = \mats \mata$.
In our case, such a matrix can be constructed by letting each
row correspond to a non-zero weight in $\weightv$.
This row in $\mats$ then has one non-zero entry equaling
to the square root of the weight.
This is similar to the method used by Clarkson and Woodruff in that
each column has at most one non-zero entry, but has the
additional property that each row has at most one non-zero entry,
that's also non-negative.



\subsection{Row Sampling Using Statistical Leverage Scores}
\label{subsec:sample}

Matrix concentration bounds can be viewed as generalizations
of single-variable concentration bounds.
To our knowledge, the first nearly-tight bounds that encapsulates
row sampling was given by Ahlswede and Winter \cite{AhlswedeW02}.
Similar bounds were given as part of a much larger set of results
by Rudelson and Vershynin \cite{RudelsonV07}, although simplifications
of their proofs are similar to previous works \cite{VershyninNotes, Harvey11notes}.
These results identified statistical leverage scores as the crucial
numbers corresponding to sampling probabilities.
Formally, the statistical leverage score of a row of $\mata$, $\veca_i$
is defined as:
\begin{align*}
\leverage_i = \veca_i \elementsum^{+} \veca_i^{T}
\end{align*}
Where $\elementsum^{+}$ is the pseudoinverse of $\elementsum$.

Although these values have been studied in statistics,
their use in algorithms is more recent.
Spielman and Srivastava used these bounds
in their spectral sparsification algorithm \cite{SpielmanS08}.
However, their algorithm was restricted to the setting where $\mata$
is the edge-vertex incidence matrix of some graph.
Works by Drineas, Mahoney, Avron and Toledo generalized this
sampling scheme to arbitrary PSD matrices \cite{DrineasM10,AvronT11}.
For our algorithms, we have crude approximations of leverage scores,
but only need to bound the number of samples.
Such extensions are immediate from the presentations given in
\cite{VershyninNotes, Harvey11notes}.
We use the statement obtained by combining Theorems 5.4. and 6.2.
from \cite{AvronT11}, as
it gives guarantees for sampling with upper bounds of leverage scores.


\begin{lemma}
\label{lem:sparsify}
(Theorem 5.4, 6.2 from \cite{AvronT11})
Let $\mata$ be a $n \times d$ matrix and $\elementsum$ be its inner product,
$\elementsum = \mata^T \mata$.
Suppose $\approxleveragev$ is a length $n$ vector such that
$\approxleverage_i \geq \leverage_i$.
Associate the probability with every row:
\begin{align}
p_i = \frac{\approxleverage_i}{||\approxleverage||_1}
\end{align}
and let $\sample_1 \ldots \sample_{M}$ be i.i.d. random matrices defined by:
\begin{align}
\sample_{i} = p_{J_i}^{-1} \element_{J_i}
\end{align}
Where $J_1 \ldots J_{M}$ are random integers between $1$ and $n$ which take
value $i$ with probability $p_i$.
Then there exist an absolute constant $C$ such that
given any error parameter $\epsilon$,
choosing $M = C ||\approxleverage||_1 \log(||\approxleverage||_1) / \epsilon^2$ gives:
\begin{align*}
\prob{(1 - \epsilon) K \preceq \frac{1}{M} \sum_{i} \sample_i \preceq (1 + \epsilon) K}
\geq & 1 -  \frac{1}{\poly(M)}
\end{align*}

Furthermore, this process, which we denote as
$\textsc{Sample}(\mata, \approxleveragev, \epsilon)$
can run in $O(n + M \log{n})$ time.
\end{lemma}

Note that the total number of sample
depends on the sum of the upper bounds.
In the case we use the exact scores, the following fact
implies about $O(d\log{d})$ samples suffice.

\begin{fact}
\label{fact:leveragesum} (see e.g. \cite{SpielmanS08})
\begin{align*}
\sum_{i = 1}^n \leverage_i = r \leq d
\end{align*}
\end{fact}

The sampling process described in Lemma \ref{lem:sparsify} is with replacement,
and is similar to the framework described in
\cite{AhlswedeW02, RudelsonV07,Harvey11notes}.
The running time can be obtained by computing partial sums of
$\approxleveragev$ and binary search for the entry where the cumulative
probability meets our threshold.
Ipsen and Wentworth showed that a variety of different sampling methods
lead to similar results both theoretically and experimentally \cite{IpsenW12}.
Since $\approxleverage_i$ only needs to be upper bounds for $\leverage_i$,
we can also use poor approximations of leverage scores by scaling them up
by the approximation factor.
This scaling leads to an increases in the number of rows sampled
by the same factor as the approximation ratio.
However, it allows us to obtain a much more accurate estimate of
$\mata$ compared to the accuracy of the approximate
statistical leverage scores.


\subsection{Generalized Stretch and Their Properties}
\label{subsec:leverageproperties}
As our algorithm is iterative and its output is approximate,
we will not be able to compute $\elementsum$ exactly.
Therefore, all the statistical leverage score estimations in our algorithms
will be done using an approximation $\elementsumapprox$
in place of $\elementsum$.
As a result, we will incorporate the matrix that we compute
these scores by, $\elementsum$ as part of our notation.
This is a common notion used in the design of combinatorial
preconditioners, where $\elementsumapprox$ is often chosen
to be a simpler matrix than $\elementsum$.
In the tree setting, Spielman and Woo \cite{SpielmanW09}
showed that when $\mata$ is an edge-vertex incidence
matrix and $\elementsumapprox$ corresponds to a spanning
tree, $\veca_i \elementsumapprox \veca_i^T$ equals to the
combinatorial stretch of the edge $i$ w.r.t. the tree.
This motivates us to use generalized stretch to
describe this term for arbitrary matrices.
Suppose we're given a factorization of $\elementsumapprox$
as $\matb^T \matb$, we will use $\str{\matb}{\veca_i}$
to denote:
\begin{align}
\str{\matb}{\veca_i}
:= \veca_i \elementsumapprox^{+} \veca_i
=  \veca_i (\matb^T \matb)^{+} \veca_i
\end{align}
Note that under this notation, the original definition of statistical
leverage score of row $i$, $\leverage_i$ equals to
$\str{\mata}{\veca_i}$.
We will also use this generalized notion to denote leverage scores
from this point and on, but still use $\approxleverage$ to denote
the approximate bounds of leverage scores computed by our algorithms.

Instead of measuring the stretch of a single row of $\mata$,
we can also incorporate the stretch of a subset of the rows
into our notation.
If $\mata$ is a matrix with $n$ rows, we use the notation
$\str{\matb}{\mata}$ to denote:
\begin{align}
\str{\matb}{\mata}
= \sum_{i = 1}^{n} \str{\matb}{\veca_{i}}
\end{align}
The following fact is also crucial for our analysis:
\begin{fact}
\label{fact:stretchclosedform}
Let $\elementsumapprox = \matb^T \matb$.
The generalized stretch of the $i^{th}$ row w.r.t $\matb$ equals to its
$L_2^2$ norm under the transformation $\elementsumapprox^{+1/2}$:
\begin{align*}
\str{\matb}{\veca_i}
=& ||\elementsumapprox^{+1/2} \veca_i^T||_2^2
= ||\veca_i \elementsumapprox^{+1/2}||_2^2
\end{align*}
and the total stretch of all rows is
\begin{align*}
\str{\matb}{\mata}
= & || \elementsumapprox^{+1/2} \mata^T||_F^2
= ||\matb \elementsumapprox^{+1/2}||_F^2
\end{align*}
Where $\elementsumapprox^{+1/2}$ is the $1/2$ power of the
pseudo-inverse of $\elementsumapprox$ and $||\cdot||_F$ denotes
the Forbenius norm.
\end{fact}

Computing stretch using a different matrix, $\str{\matb}{\mata}$,
is a standard step when analyzing graph based preconditioners,
and done implicitly in \cite{KoutisLP12}.
It was shown by Avron, Maymounkov and Toledo that similar
matrices can be used in place of each other in least squares
regression \cite{AvronMT10}.
The same also holds for generalized stretch, where
similar matrices can be used to approximate stretch
up to the same factor as their difference.
This allows us to define the notion of $S$-stretch base.

\begin{definition}
\label{def:lowstretch}
A matrix $\matb$ is a $S$-stretch base for $\mata$ if:
\begin{enumerate}
	\item \label{part:pointwise}
		$\str{\matb}{\veca_i} \geq \leverage_i$
	\item \label{part:total}
		$\str{\matb}{\mata} \leq S$
\end{enumerate}
\end{definition}

This definition is similar to the objective of the column
subset selection problem studied by Avron and Boutsidis \cite{AvronB12}.
Its two conditions are consequences of the requirements
on sampling probabilities described in Lemma \ref{lem:sparsify}.
Condition \ref{part:pointwise} implies
that $\str{\mata}{\veca_i}$ can be used
as sampling probabilities;
while condition \ref{part:total} means if $\kappa = \poly(d)$,
the total number of rows needed for a constant error
can be bounded by $O(\kappa d \log{d})$.
Works on spectral sparsifiers of graphs showed
that matrices similar to $\mata$, $\matb$, can still lead
to sampling probabilities \cite{SpielmanS08, KoutisLP12}.
One sufficient condition is that $\matb^T \matb$ is spectrally
close to $\mata^T \mata$.
It can be formalized using Definition \ref{def:lowstretch}
as follows:
\begin{lemma}
\label{lem:baseswitch}
For fixed $\mata$ and $\elementsum = \mata^T \mata$,
if $\elementsumapprox = \matb^T \matb$ satisfies:
\begin{align*}
\frac{1}{\kappa} \elementsum
\preceq & \elementsumapprox
\preceq \elementsum
\end{align*}
Then $\matb$
is a $\kappa$-stretch base for $\mata$.
\end{lemma}
Using different bases play crucial roles in
both of our algorithms described in Sections
\ref{sec:simple} and \ref{sec:rowcombine}.




\subsection{Estimation of Generalized Stretch}
\label{subsec:estimatestretch}

Fact \ref{fact:stretchclosedform} shows that
gives that $\str{\mata}{\veca_i}$
is the $L_2$ norm of a vector.
Combining this norm using the Johnson-Lindenstrauss transform
(e.g. \cite{Achlioptas01}) the leads to faster approximations
of all leverage scores.
This was first used by Spielman and Srivastava to approximate
effective resistances \cite{SpielmanS08}.
Direct applications of this reduction, or similar algorithms
given in \cite{DrineasMMW11} lead to a running time of
at least $\Omega(\nnz(\mata) \log{n})$.
However, the definition of generalized stretch are only
one sided bounds pointwise, which means our estimates
can also have large, one sided error.
We can use fewer vectors in the projection, and scale up
the results to correct potential underestimates.
This trades off the coefficient on the leading term at the
cost of more elements sampled.
This way of remedying one-sided error in the Johnson-Lindenstrauss
transform was first shown in \cite{KoutisLP12} and relies on a version
of the projection theorem with fewer vectors.
We use the following version given as Lemma 7 in \cite{IndykM98}:

\begin{lemma}
\label{lem:jl} (Lemma 7 from \cite{IndykM98})
Let $u$ be a unit vector in $\Re^\nu$.
For any given positive integers $k$, let $U_1, \ldots, U_k$ be random vectors
chosen independently from the $\nu$-dimensional Gaussian distribution $N^\nu(0, 1)$.
For $X_i = u^T U_i$, define $W = W(u) = (X_1, \ldots, X_k)$ and
$L = L(u) = \|W\|^2_2$. Then for any $\beta > 1$:
\begin{enumerate}
    \item \label{part:expectation}
		$E(L) = k$
    \item \label{part:upper}
		$\prob{L \geq \beta k} < O(k)  \exp(-\frac{k}{2} (\beta - (1 + \ln{\beta})) )$
    \item \label{part:lower}
		$\prob{L \leq k / \beta} < O(k)  \exp(-\frac{k}{2} (\beta^{-1} - (1 - \ln{\beta})) )$
\end{enumerate}
\end{lemma}

The other observation needed to apply this lemma is that
$\elementsumapprox^{+1/2}$ from Fact \ref{fact:stretchclosedform}
can be replaced by any matrix whose product with its
transpose equals to $\elementsumapprox$.
As $\elementsumapprox = \matb^T \matb$,\
$\elementsumapprox^{+}
= \elementsumapprox^{+} \matb^T \matb \elementsumapprox^{+}
= (\matb \elementsumapprox^{+})^T \matb \elementsumapprox^{+}$.
Using this matrix in place of $\elementsumapprox^{+1/2}$ avoids  
computing the $1/2$ power of $\elementsumapprox$.
Pseudocode of our estimation algorithm is shown in Algorithm
\ref{alg:approxstretch},
while the error analysis is nearly identical to the ones given in
Section 4 of \cite{SpielmanS08} and Section 3.2. of \cite{DrineasMMW11}.


\begin{algo}[ht]
\qquad

$\textsc{ApproxStr}(\mata, \matb, \beta, \delta)$
\vspace{0.05cm}

\underline{Input:}
Matrix $\mata$, approximation $\matb$ such that
$\matb^T \matb$ is a $\kappa$-stretch base for $\mata$,
value $\kappa$,
parameter $\beta$ indicating allowed estimation error.
Failure probability $\delta$.

\underline{Output:}
Upper bounds for stretches of rows of $\mata$
measured w.r.t. $\elementsumapprox$:
$\approxleverage_1 \ldots \approxleverage_n$.

\begin{algorithmic}
\STATE{Compute $\elementsumapprox = \matb^T \matb$}
\STATE{Compute $\elementsum^{+}$}
\STATE{Let $k = O(\log_{\beta} (1 / \delta))$}
\STATE{Let $\matu$ be a $k \times n$ matrix with
	each entry is picked independently from $N(0, 1)$}
\STATE{Let $\approxleverage_i$ be $\frac{\beta}{k} ||\matu \mataapprox \elementsumapprox^{+} \veca_i^T||_2^2$.}
\RETURN{$\approxleveragev$}
\end{algorithmic}

\caption{Algorithm for Upper Bounding Stretch}

\label{alg:approxstretch}
\end{algo}

\begin{lemma}
\label{lem:approxstretchjl}
For each $i$, with probability at least $1 - \delta$ we have:
\begin{align*}
||\matu \mataapprox \elementsumapprox^{+} \veca_i^T||_2^2
\geq \frac{1}{\beta}  \str{\elementsumapprox}{\veca_i}
\end{align*}
\end{lemma}

\Proof
%of{Lemma \ref{lem:approxstretchjl}}
We can rewrite $\elementsumapprox^{+}$ as
$\elementsumapprox^{+} \mataapprox^T \mataapprox \elementsumapprox^{+}$ to get:
\begin{align}
\leveragescore{\elementsumapprox}{\veca_i}
= & \veca_i \elementsumapprox^{+} \veca_i^T \nonumber \\
= & \veca_i \elementsumapprox^{+} \elementsumapprox
	\elementsumapprox^{+}  \veca_i^T \nonumber \\
= & \veca_i \elementsumapprox^{+} (\mataapprox^T \mataapprox)
	\elementsumapprox^{+}  \veca_i^T \nonumber \\
= & \veca_i \elementsumapprox^{+} \mataapprox^T
	\mataapprox \elementsumapprox^{+} \veca_i^T \nonumber \\
= & ||\mataapprox \elementsumapprox^{+} \veca_i^T||_2^2
\end{align}
By Lemma \ref{lem:jl} Part \ref{part:lower} we have:
\begin{align}
& \Pr \left[\frac{1}{k} ||\matu \mataapprox \elementsumapprox^{+}\veca_i^T||_2^2 < \frac{1}{\beta} ||\mataapprox \elementsumapprox^{+}\veca_i^T||_2^2 \right] \nonumber \\
\leq & \exp\left(-\frac{k}{2} (\beta^{-1} - (1 - \ln{\beta})) \right)\nonumber \\
\leq & \exp\left(-\frac{k}{2} (\ln{\beta} - 1) \right) \nonumber\\
\leq & \exp\left(-\frac{k}{2} \frac{\ln{\beta}}{2} \right)
= \beta^{-\frac{k}{4}}
\end{align}
By a suitable choice of constants in $k = O(\log_{\beta}{(1/\delta)})$ this can
be made less than $\delta$.
\QED




Bounding the total of $\approxleverage_i$, as well as
the running time gives the following guarantees about
\textsc{ApproxStr}:

\begin{lemma}
\label{lem:approxstretch}
Let $\mata$ be a $n \times d$ matrix, and
$\matb$ an approximation with $\tilde{n}$ rows such that
$\elementsumapprox = \matb^T \matb$
is a $\kappa$-stretch base for $\mata$.
Then $\textsc{ApproxStr}(\mata, \matb, \beta, \delta)$ runs in
$O( (\nnz(A) + \nnz(\mataapprox) + d^{2} ) \log_{\beta}{(1 / \delta)} 
+ (\tilde{n} + d) d^{\omega - 1} \log{d} \epsilon^{-2})$ time
returns upper bounds $\approxleverage_i$ such that:
\begin{enumerate}
\item \label{part:jlupper} For each $i$, with probability at least
$1 - \delta$ we have $\approxleverage_i \geq \leverage_i$
\item \label{part:jlsum} $||\approxleverage||_1 \leq O(\beta \kappa d \log{(1/\delta)})$ with
probability at least $1 - \delta$.
\end{enumerate}
\end{lemma}

\Proof
Lemma \ref{lem:approxstretchjl} gives
\begin{align*}
||\matu \mataapprox \elementsumapprox^{+} \veca_i^T||_2^2
\geq \frac{1}{\beta}  \leveragescore{\elementsumapprox}{\veca_i}
\end{align*}
This and Part \ref{part:pointwise} of Definition \ref{def:lowstretch}
means scaling the estimates up by a factor of $\beta$ suffices
to give upper bounds of the leverage scores.
The upper bound on $\sum_{i} \approxleverage_i$ then can be obtained
similar to the proof of Lemma \ref{lem:approxstretchjl},
along with the bound on $\str{\elementsumapprox}{mata}$
given in Part \ref{part:upper} of Lemma \ref{lem:jl}.

Note that:
\begin{align}
\sum_{i} \approxleverage_i
= & \frac{\kappa \beta}{k} ||\matu \mataapprox \elementsumapprox^{+} \veca_i^T||_2^2 \nonumber \\
= & \frac{\kappa \beta}{k} ||\matu \mataapprox \elementsumapprox^{+} \mata^T||_F^2
\end{align}
Let $\vecy$ be the vector that's the row norms of
$\matb \elementsumapprox^{+} \mata$.
Note that 
$||y||_2^2
= \sum_{i=1}^{n} ||\matb \elementsumapprox^{+} \veca_i^T||_2^2 \nonumber \\
= \str{\elementsumapprox}{\mata} \leq \kappa d$,
where the last inequality follows from
Part \ref{part:total} of Definition \ref{def:lowstretch}.
Part \ref{part:upper} of Lemma \ref{lem:jl} can be used to
bound $\frac{1}{k} ||\matu \vecy||_2^2$.
Note that when $t > 10$, $t - 1 - \ln{t} \geq t / 2$.
If $k$ is larger than some absolute constant, this gives:
\begin{align}
& \prob{\frac{1}{k} ||\matu \vecy||_2^2
> \beta \kappa d \geq \log(1/\delta) ||\vecy||_2^2} \nonumber \\
\leq & O \left( k \exp(-\frac{k}{2} \frac{\log(1/\delta)}{2} ) \right)
\leq \delta
\end{align}

It remains to bound the running time of $\textsc{LeverageUpper}$.
Finding $\elementsum$ takes $O(\tilde{n} d^{\omega - 1})$ time,
while inverting it takes an additional $d^{\omega}$ time.
Computing $\matu \mataapprox$ can be done in $O(\nnz(\mataapprox)k)$ time,
and multiplying it on the right by $\elementsum^{+}$ to
obtain $\matu \mataapprox \elementsumapprox^{+}$ takes $O(kd^2)$ time.
It remains to evaluate
$\matu \mataapprox \elementsumapprox^{+} \veca_i^T$
for each row $i$.
This can be done by summing $\nnz(\veca_i)$ length $k$ vectors,
giving a total of $\nnz(\mata) k$ over all $n$ vectors.
Therefore the total cost for computing the estimates is
$O(k(\nnz(\mata) + \nnz(\mataapprox) + d^2) + (\tilde{n} + d)d^{\omega - 1})$.
\QED

